CoCAI: Copula-based Conformal Anomaly Identification for Multivariate Time-Series

We propose a novel framework that harnesses the power of generative artificial intelligence and copula-based modeling to address two critical challenges in multivariate time-series analysis: delivering accurate predictions and enabling robust anomaly detection. Our method, Copula-based Conformal Anomaly Identification for Multivariate Time-Series (CoCAI), leverages a diffusion-based model to capture complex dependencies within the data, enabling high quality forecasting. The model's outputs are further calibrated using a conformal prediction technique, yielding predictive regions which are statistically valid, i.e., cover the true target values with a desired confidence level. Starting from these calibrated forecasts, robust outlier detection is performed by combining dimensionality reduction techniques with copula-based modeling, providing a statistically grounded anomaly score. CoCAI benefits from an offline calibration phase that allows for minimal overhead during deployment and delivers actionable results rooted in established theoretical foundations. Empirical tests conducted on real operational data derived from water distribution and sewerage systems confirm CoCAI's effectiveness in accurately forecasting target sequences of data and in identifying anomalous segments within them.

==> tables/union.tex <==
\begin{table}[!h]

\centering
\caption{Comparison of the average width and data coverage percentage between the Empirical Quantile Range (EQR) and conformalized intervals across the considered datasets. The results highlight superior coverage for the conformalized interval, while only requiring minor adjustments.
}\label{tab:intervals}
\adjustbox{max width=\linewidth}{
\begin{tabular}{lcc|cc|cc|}
\cline{4-7}
                                     &                             &              & \multicolumn{2}{c|}{\textbf{EQR}}                 & \multicolumn{2}{c|}{\textbf{Conformalized Interval}}                    \\ \cline{2-7} 
\multicolumn{1}{l|}{}                & \multicolumn{1}{c|}{Obs} & Median Value & \multicolumn{1}{c|}{Avg. Width} & Coverage (\%)                        & \multicolumn{1}{c|}{Avg. Width} & Coverage (\%)                         \\ \hline
\multicolumn{1}{l|}{Sew. - Level}    & \multicolumn{1}{c|}{1295}   & 0.452        & \multicolumn{1}{c|}{0.008}      & {\color[HTML]{FE0000} \textbf{1.62}} & \multicolumn{1}{c|}{0.026}      & {\color[HTML]{009901} \textbf{91.58}} \\
\multicolumn{1}{l|}{Sew. - Speed}    & \multicolumn{1}{c|}{1301}   & 0.358        & \multicolumn{1}{c|}{0.024}      & {\color[HTML]{FE0000} \textbf{2.77}} & \multicolumn{1}{c|}{0.058}      & {\color[HTML]{009901} \textbf{90.70}} \\
\multicolumn{1}{l|}{WDS - Flow-rate} & \multicolumn{1}{c|}{1613}   & 53.27        & \multicolumn{1}{c|}{2.82}       & {\color[HTML]{FE0000} \textbf{0.25}} & \multicolumn{1}{c|}{7.14}       & {\color[HTML]{009901} \textbf{90.45}} \\
\multicolumn{1}{l|}{WDS - Pressure}  & \multicolumn{1}{c|}{1604}   & 7.50         & \multicolumn{1}{c|}{0.03}       & {\color[HTML]{FE0000} \textbf{2.24}} & \multicolumn{1}{c|}{0.07}       & {\color[HTML]{009901} \textbf{89.29}} \\ \hline
\end{tabular} 
}

%\end{table}

%\begin{table}[!b]



\caption{Comparison of flagging rates for both Gaussian and Student's t Copula models while also accounting for conformalized interval coverage rates over the considered datasets. Results for series which are not flagged are also show.}
\label{tab:copula}
\adjustbox{max width=\linewidth}{
\begin{tabular}{lcc|cc|ccc|cc}
\multicolumn{1}{c}{}                 &                                                                       &                                                     & \multicolumn{2}{c|}{\textbf{$\mathbf{a_G > 0.9}$}}                                                                               & \multicolumn{3}{c|}{\textbf{$\mathbf{a_S > 0.9}$}}                                                                                                             & \multicolumn{2}{c}{\textbf{$\mathbf{a_G \leq 0.9 \wedge a_S \leq 0.9}$}}                                                                              \\ \cline{2-10} 
\multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\#\\ obs\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\# \\ basis\end{tabular} & \begin{tabular}[c]{@{}c@{}}Inside\\ Interval (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Outside\\ Interval (\%)\end{tabular} & \multicolumn{1}{c|}{$\nu$} & \begin{tabular}[c]{@{}c@{}}Inside\\ Interval (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Outside\\  Interval (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Inside\\ Interval (\%)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Outside\\ Interval (\%)\end{tabular}} \\ \hline
\multicolumn{1}{l|}{Sew. - Level}    & \multicolumn{1}{c|}{1295}                                             & 15                                                  & \begin{tabular}[c]{@{}c@{}}110\\ (8.49)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}73\\ (5.64)\end{tabular}             & \multicolumn{1}{c|}{25}    & \begin{tabular}[c]{@{}c@{}}79\\ (6.10)\end{tabular}            & \begin{tabular}[c]{@{}c@{}}63\\ (4.86)\end{tabular}              & \begin{tabular}[c]{@{}c@{}}1076\\ (83.09)\end{tabular}         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}36\\ (2.78)\end{tabular}}             \\ \hline
\multicolumn{1}{l|}{Sew. - Speed}    & \multicolumn{1}{c|}{1301}                                             & 13                                                  & \begin{tabular}[c]{@{}c@{}}119\\ (9.15)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}89\\ (6.84)\end{tabular}             & \multicolumn{1}{c|}{20}    & \begin{tabular}[c]{@{}c@{}}73\\ (5.61)\end{tabular}            & \begin{tabular}[c]{@{}c@{}}76\\ (5.84)\end{tabular}              & \begin{tabular}[c]{@{}c@{}}1061\\ (81.55)\end{tabular}         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}32\\ (2.46)\end{tabular}}             \\ \hline
\multicolumn{1}{l|}{WDS - Flow-rate} & \multicolumn{1}{c|}{1613}                                             & 15                                                  & \begin{tabular}[c]{@{}c@{}}163\\ (10.11)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}85\\ (5.27)\end{tabular}             & \multicolumn{1}{c|}{11}    & \begin{tabular}[c]{@{}c@{}}91\\ (5.64)\end{tabular}            & \begin{tabular}[c]{@{}c@{}}70\\ (4.34)\end{tabular}              & \begin{tabular}[c]{@{}c@{}}1293\\ (80.16)\end{tabular}         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}68\\ (4.22)\end{tabular}}             \\ \hline
\multicolumn{1}{l|}{WDS - Pressure}  & \multicolumn{1}{c|}{1604}                                             & 15                                                  & \begin{tabular}[c]{@{}c@{}}105\\ (6.55)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}73\\ (5.55)\end{tabular}             & \multicolumn{1}{c|}{23}    & \begin{tabular}[c]{@{}c@{}}72\\ (4.49)\end{tabular}            & \begin{tabular}[c]{@{}c@{}}66\\ (4.11)\end{tabular}              & \begin{tabular}[c]{@{}c@{}}1327\\ (82.73)\end{tabular}         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}99\\ (6.17)\end{tabular}}             \\ \hline
\end{tabular}
}

\end{table}

